On Central Primitives for Quantum Cryptography with Classical Communication

Recent work has introduced the "Quantum-Computation Classical-Communication" (QCCC) (Chung et. al.) setting for cryptography. There has been some evidence that One Way Puzzles (OWPuzz) are the natural central cryptographic primitive for this setting (Khurana and Tomer). For a primitive to be considered central it should have several characteristics. It should be well behaved (which for this paper we will think of as having amplification, combiners, and universal constructions); it should be implied by a wide variety of other primitives; and it should be equivalent to some class of useful primitives. We present combiners, correctness and security amplification, and a universal construction for OWPuzz. Our proof of security amplification uses a new and cleaner version construction of EFI from OWPuzz (in comparison to the result of Khurana and Tomer) that generalizes to weak OWPuzz and is the most technically involved section of the paper. It was previously known that OWPuzz are implied by other primitives of interest including commitments, symmetric key encryption, one way state generators (OWSG), and therefore pseudorandom states (PRS). However we are able to rule out OWPuzz's equivalence to many of these primitives by showing a black box separation between general OWPuzz and a restricted class of OWPuzz (those with efficient verification, which we call EV-OWPuzz). We then show that EV-OWPuzz are also implied by most of these primitives, which separates them from OWPuzz as well. This separation also separates extending PRS from highly compressing PRS answering an open question of Ananth et. al.

==> concurrent.tex <==
\section{Concurrent Work}

Two concurrent works~\cite{prssep,sigsep} also produced black-box separations of QCCC primitives from linear output pseudorandom states.

~\cite{prssep} shows that if QCCC pseudodeterministic one-way functions exist, then $\BQP\neq \QCMA$. Since by~\cite{Kretschmer21Quantum}, there exists an oracle relative to which linear output pseudorandom states exist and $\BQP = \QCMA$, this gives a black-box separation of pseudodeterministic one-way functions from pseudorandom states. In addition, pseudodeterministic one-way functions can be built from pseudodeterministic PRGs, which in turn can be built from pseudorandom states with logarithmic output length. Thus,~\cite{prssep} gives a black-box barrier against length extension for pseudorandom states.

In comparison, our black-box separation shows that if efficiently verifiable one-way puzzles exist, then $\BQP\neq \QCMA$. It is easy to see that efficiently verifiable one-way puzzles can be built from pseudodeterministic one-way functions, and so the results of~\cite{prssep} follow as a corollary of our~\Cref{thm:separation}. 

~\cite{sigsep} shows that many-time signatures with quantum verification key and classical signature/signing key cannot be built in a black-box manner from pseudorandom states. In particular, they define a novel oracle (using similar techniques to~\cite{Kretschmer21Quantum}) under which linear output pseudorandom states exist and such many-time signature schemes do not. Since a signature scheme of this type can be built from logarithmic output pseudorandom states~\cite{botprfs}, this again gives a black-box barrier against length extension for pseudorandom states. Their result is also interesting since one-time signatures with quantum verification key and classical signature/signing key \textit{can} be built from pseudorandom states~\cite{moryam22}. Thus, this gives a black-box separation between one-time and many-time security for such signature schemes.

Note that entirely QCCC signatures (with classical verification key) can be used to build efficiently verifiable one-way puzzles~\cite{khurana2024commitments}. Thus, our~\Cref{thm:separation} gives a barrier towards building QCCC signatures from pseudorandom states. However, our techniques do not apply when the verification key is quantum, and~\cite{sigsep}'s solution for this requires significant technical work.

In comparison to both of these results, our black-box separation has the advantage that it is fairly general. Efficiently verifiable one-way puzzles can be built from most QCCC cryptographic primitives (see~\Cref{thm:reductions}). And so our separation gives a barrier against building any of these QCCC primitives from pseudorandom states (or inefficiently verifiable one-way puzzles).

